Taming the Curse of Dimensionality: Discrete Integration by Hashing and Optimization

Integration is affected by the curse of dimensionality and quickly becomes intractable as the dimensionality of the problem grows. We propose a randomized algorithm that, with high probability, gives a constant-factor approximation of a general discrete integral defined over an exponentially large set. This algorithm relies on solving only a small number of instances of a discrete combinatorial optimization problem subject to randomly generated parity constraints used as a hash function. As an application, we demonstrate that with a small number of MAP queries we can efficiently approximate the partition function of discrete graphical models, which can in turn be used, for instance, for marginal computation or model selection.

==> Makefile <==
.PHONY: main fromscratch dvi ps pdf bibs figs compact clean

TEXFILE    = whcount

LATEX      = latex
BIBTEX     = bibtex
PDFLATEX   = pdflatex
PSTOPDF    = ps2pdf
DVIPS      = dvips -T 8.5in,11in
FIGDIR     = figs
CURRENTDIR = `basename "\`pwd\`"`

default: pdf

#fromscratch: figs
fromscratch:
	$(LATEX) $(TEXFILE)
	$(BIBTEX) $(TEXFILE)
	$(LATEX) $(TEXFILE)
	$(LATEX) $(TEXFILE)
	$(DVIPS) $(TEXFILE).dvi -o $(TEXFILE).ps

dvi:
	$(LATEX) $(TEXFILE)

ps: dvi
	$(DVIPS) $(TEXFILE).dvi -o $(TEXFILE).ps

pdf:
	$(PDFLATEX) $(TEXFILE)

#pdf: ps
#	$(PSTOPDF) $(TEXFILE)

bibs:
	$(BIBTEX) $(TEXFILE)

figs:
	(cd $(FIGDIR); bash ./makefigs ../*.tex )

compact:
	(rm -f $(TEXFILE).{aux,log,blg,out,toc} )

clean: compact
	(rm -f $(TEXFILE).{dvi,ps,pdf} )


